Connecting Distributed Pockets of EnergyFlexibility through Federated Computations:Limitations and Possibilities

Electric grids are traditionally operated as multi-entity systems with each entity managing a geographical region. Interest and demand for decarbonization and energy democratization is resulting in growing penetration of controllable energy resources. In turn, this process is increasing the number of grid entities. The paradigm shift is also fueled by increased adoption of intelligent sensors and actuators equipped with advanced processing and computing capabilities. While collaboration among power grid entities (agents) reduces energy cost and increases overall reliability, achieving effective collaboration is challenging. The main challenges stem from the heterogeneity of system agents and their collected information. Furthermore, the scale of data collection is constantly increasing and many grid entities have strict privacy requirements. Another challenge is the energy industry's common practice of keeping data in silos. Federated computation is an approach well suited to addressing these issues that are increasingly important for multi-agent energy systems. Through federated computation, agents collaboratively solve learning and optimization problems while respecting each agent's privacy and overcoming barriers of cross-device and cross-organization data isolation. In this paper, we first establish the need for federated computations to achieve energy optimization goals of the future power grid. We discuss practical challenges of performing multi-agent data processing in general. Then we address challenges that arise specifically for orchestrating operation of connected distributed energy resources in the Internet of Things. We conclude this paper by presenting a novel federated computation framework that addresses some of these issues, and we share examples of two initial field test setups in research demonstrations and commercial building applications with Grid Fruit LLC.

==> FL4harvesting.tex <==
\subsection{underlying needs}
\subsection{disruption potentials}


==> bibliography/output.tex <==
% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Delgado2018}
\BIBentryALTinterwordspacing
J.~Delgado, R.~Faria, P.~Moura, and A.~de~Almeida, ``Impacts of plug-in
  electric vehicles in the portuguese electrical grid,'' \emph{Transportation
  Research Part D: Transport and Environment}, vol.~62, pp. 372 -- 385, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.trd.2018.03.005}
\BIBentrySTDinterwordspacing

\bibitem{RNC2050}
Portugal, ``Roadmap for carbon neutrality 2050,'' Portuguese Republic, Tech.
  Rep., 2019.

\bibitem{moura2020linking}
P.~Moura, G.~Yu, S.~Sarkar, and J.~Mohammadi, ``Linking parking and electricity
  values to unlock potentials of electric vehicles in portuguese buildings,''
  in \emph{PES General Meeting}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2020.

\bibitem{Gray2018}
\BIBentryALTinterwordspacing
M.~K. {Gray} and W.~G. {Morsi}, ``A novel transactive energy framework for
  prosumers with battery storage and electric vehicles,'' in \emph{2018 IEEE
  Electrical Power and Energy Conference (EPEC)}, Oct 2018, pp. 1--6. [Online].
  Available: \url{https://doi.org/10.1109/EPEC.2018.8598368}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019b}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, K.~{Ma}, M.~{Shahidehpour}, Y.~{Xue}, and S.~{Huang},
  ``Two-stage optimal scheduling of electric vehicle charging based on
  transactive control,'' \emph{IEEE Transactions on Smart Grid}, vol.~10,
  no.~3, pp. 2948--2958, May 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2815593}
\BIBentrySTDinterwordspacing

\bibitem{Jin2017}
\BIBentryALTinterwordspacing
X.~Jin, J.~Wu, Y.~Mu, M.~Wang, X.~Xu, and H.~Jia, ``Hierarchical microgrid
  energy management in an office building,'' \emph{Applied Energy}, vol. 208,
  pp. 480 -- 494, 2017. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2017.10.002}
\BIBentrySTDinterwordspacing

\bibitem{Thomas2018}
\BIBentryALTinterwordspacing
D.~Thomas, O.~Deblecker, and C.~S. Ioakimidis, ``Optimal operation of an energy
  management system for a grid-connected smart building considering
  photovoltaics’ uncertainty and stochastic electric vehicles’ driving
  schedule,'' \emph{Applied Energy}, vol. 210, pp. 1188 -- 1206, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.apenergy.2017.07.035}
\BIBentrySTDinterwordspacing

\bibitem{Nefedov2018}
\BIBentryALTinterwordspacing
E.~Nefedov, S.~Sierla, and V.~Vyatkin, ``Internet of energy approach for
  sustainable use of electric vehicles as energy storage of prosumer
  buildings,'' \emph{Energies}, vol.~11, no.~8, 2018. [Online]. Available:
  \url{https://doi.org/10.3390/en11082165}
\BIBentrySTDinterwordspacing

\bibitem{Quddus2018}
\BIBentryALTinterwordspacing
M.~A. Quddus, O.~Shahvari, M.~Marufuzzaman, J.~M. Usher, and R.~Jaradat, ``A
  collaborative energy sharing optimization model among electric vehicle
  charging stations, commercial buildings, and power grid,'' \emph{Applied
  Energy}, vol. 229, pp. 841 -- 857, 2018. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2018.08.018}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, M.~{Shahidehpour}, C.~{Li}, S.~{Huang}, and W.~{Wei},
  ``Transactive real-time electric vehicle charging management for commercial
  buildings with pv on-site generation,'' \emph{IEEE Transactions on Smart
  Grid}, vol.~10, no.~5, pp. 4939--4950, Sep. 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2871171}
\BIBentrySTDinterwordspacing

\bibitem{Fonseca2018}
\BIBentryALTinterwordspacing
P.~{Fonseca}, P.~{Moura}, H.~{Jorge}, and A.~T. {de Almeida}, ``Sustainability
  in university campus: options for achieving nearly zero energy goals,''
  vol.~19, no.~4, pp. 790--816, Jan. [Online]. Available:
  \url{https://doi.org/10.1108/IJSHE-09-2017-0145}
\BIBentrySTDinterwordspacing

\bibitem{mohammadi2019collaborative}
\BIBentryALTinterwordspacing
J.~Mohammadi and S.~Kolouri, ``Collaborative learning through shared collective
  knowledge and local expertise,'' in \emph{29th International Workshop on
  Machine Learning for Signal Processing}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2019. [Online]. Available:
  \url{https://doi.org/10.1109/MLSP.2019.8918888}
\BIBentrySTDinterwordspacing

\end{thebibliography}

